A Regularized Factor-augmented Vector Autoregressive Model

We propose a regularized factor-augmented vector autoregressive (FAVAR) model that allows for sparsity in the factor loadings. In this framework, factors may only load on a subset of variables which simplifies the factor identification and their economic interpretation. We identify the factors in a data-driven manner without imposing specific relations between the unobserved factors and the underlying time series. Using our approach, the effects of structural shocks can be investigated on economically meaningful factors and on all observed time series included in the FAVAR model. We prove consistency for the estimators of the factor loadings, the covariance matrix of the idiosyncratic component, the factors, as well as the autoregressive parameters in the dynamic model. In an empirical application, we investigate the effects of a monetary policy shock on a broad range of economically relevant variables. We identify this shock using a joint identification of the factor model and the structural innovations in the VAR model. We find impulse response functions which are in line with economic rationale, both on the factor aggregates and observed time series level.

==> A_Figures_different_p12.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[H]
%	\centering
%	\includegraphics[width=1\linewidth]{irf_per_4_0}
%	\caption{{\textbf{Impulse responses for the regularized FAVAR}} \label{fig:irf_per_4_0_p3}\\
%		\footnotesize The graph shows impulse responses to an unit shock in the innovation of the FFR. The dashed lines correspond to 68\% bootstrap confidence intervals. The impulse responses are based on a FAVAR(3) model.}
%\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[H]
	\centering
	\includegraphics[width=1\linewidth]{irf_per_4_1}
	\caption{{Accumulated impulse responses to a monetary policy shock on the factors for the regularized FAVAR} \label{fig:irf_per_4_1_p12}\\
		\footnotesize The graph shows accumulated impulse responses to a 100bp shock in the innovation of the FFR. The dashed lines correspond to 68\% bootstrap confidence intervals. The impulse responses are based on a RFAVAR(12) model.}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[H]
%	\centering
%	\includegraphics[width=1\linewidth]{irf_x_per_4_0}
%	\caption{{\textbf{Impulse responses on the observed variables $x_t$ for the regularized FAVAR}} \label{fig:irf_x_per_4_0_p3}\\
%		\footnotesize The graph shows impulse responses to an unit shock in the innovation of the FFR. The dashed lines correspond to 68\% bootstrap confidence intervals. The impulse responses are based on a FAVAR(3) model.}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{1cm}

\begin{figure}[H]
	
	\centering
	\includegraphics[width=1\linewidth]{irf_x_per_4_1}
	\caption{{Accumulated impulse responses to a monetary policy shock on the observed variables $x_t$ for the regularized FAVAR} \label{fig:irf_x_per_4_1_p12}\\
		\footnotesize The graph shows accumulated impulse responses to a 100bp shock in the innovation of the FFR. The dashed lines correspond to 68\% bootstrap confidence intervals. The impulse responses are based on a RFAVAR(12) model.}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
